Analysis and approximation of mixed-dimensional PDEs on 3D-1D domains coupled with Lagrange multipliers

Coupled partial differential equations defined on domains with different dimensionality are usually called mixed dimensional PDEs. We address mixed dimensional PDEs on three-dimensional (3D) and one-dimensional domains, giving rise to a 3D-1D coupled problem. Such problem poses several challenges from the standpoint of existence of solutions and numerical approximation. For the coupling conditions across dimensions, we consider the combination of essential and natural conditions, basically the combination of Dirichlet and Neumann conditions. To ensure a meaningful formulation of such conditions, we use the Lagrange multiplier method, suitably adapted to the mixed dimensional case. The well posedness of the resulting saddle point problem is analyzed. Then, we address the numerical approximation of the problem in the framework of the finite element method. The discretization of the Lagrange multiplier space is the main challenge. Several options are proposed, analyzed and compared, with the purpose to determine a good balance between the mathematical properties of the discrete problem and flexibility of implementation of the numerical scheme. The results are supported by evidence based on numerical experiments.

==> domain.tex <==
%\documentclass{standalone}

%\usepackage{tikz}
%\usetikzlibrary{shapes, snakes, patterns, arrows}
%\usetikzlibrary{calc}
%\usepackage{pgfplots}
%\usepgfplotslibrary{fillbetween}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsfonts}

%\begin{document}
\begin{tikzpicture}


% Omega
\draw[] (0, 3) ellipse (2. and 0.5);
\draw (-2.,3) -- (-2.,-3);
\draw (-2.,-3) arc (180:360:2. and 0.5);
\draw [dashed] (-2.,-3) arc (180:360:2. and -0.5);
\draw (2.,-3) -- (2., 3);
% Top whole
\draw[blue, thick] (-0.75, 3) ellipse (0.6 and 0.15);
% Bottom whole
\draw[blue, thick] (0.75, -3) ellipse (0.6 and 0.15);
% Auxliary middle surface
\draw [dashed, thin](-2., 0) arc (180:360:2. and 0.5);
\draw [dashed, thin] (-2.,0) arc (180:360:2. and -0.5);

\fill[pattern color=cyan, pattern=north east lines] (0.5, 0) ellipse (0.5 and 0.125);
\node [cyan, below right, fill=white, opacity=0.8] at (0.6, 0.0) {\rotatebox{90}{\Large{$\mathcal{D}(s)$}}};

\node[mark size=1.5pt, color=red] at (0.5, 0.0) {\pgfuseplotmark{*}};


% Walls of gamma
\draw [blue, thick, name path global = topleft] plot [smooth, tension=1] coordinates { (-1.35,3) (-0.6, 1) (0,0)};
\draw [blue, thick, name path global = botleft] plot [smooth, tension=1] coordinates { (0,0) (0.125, -1) (0.15,-3)};

\draw [blue, thick, name path global = topright] plot [smooth, tension=1] coordinates { (-0.15,3) (0.5, 1) (1.0,0)};
\draw [blue, thick, name path global = botright] plot [smooth, tension=1] coordinates { (1.0,0) (1.25, -1) (1.35,-3)};

%\fill [gray, opacity=0.5] (-1.25,0) -- (-1.25,-3.5) arc (180:360:1.25 and 0.5) -- (1.25,0) arc (0:180:1.25 and -0.5);

\tikzfillbetween[of=topleft and topright]{blue!40!white, opacity=0.2};
\tikzfillbetween[of=botleft and botright]{blue!40!white, opacity=0.2};
\fill[blue!40!white, opacity=0.2] (-1.35, 3) arc (180:360:0.6 and -0.15) -- (-0.75, 3);
\fill[blue!40!white, opacity=0.2] (0.15, -3) arc (180:360:0.6 and 0.15) -- (-0.15, -3);
\node[blue, fill=white, opacity=0.7, above] at (1.15, -3) {\rotatebox{90}{\Large{$\Omega_{\ominus}$}}};

% Curve
\draw [very thick, red] plot [smooth, tension=0.2] coordinates { (-0.75,3) (-0.2, 1.5) (0.5, 0) (0.75,-3)};
\node[red, fill=white, opacity=0.7] at (0.075, 1) {\rotatebox{90}{\Large{$\Lambda$}}};

\node[] at (-0.5, -1.5) {\rotatebox{90}{\Large{$\Omega_{\oplus}$}}};

\node[blue] at (0.75, 1) {\rotatebox{90}{\Large{$\Gamma$}}};

\draw [very thick, cyan] (0, 0) arc (180:360:0.5 and 0.125);
\draw [very thick, dashed, cyan] (0,0) arc (180:360:0.5 and -0.125);
\node [left, cyan] at (0, 0) {\rotatebox{90}{\Large{$\partial\mathcal{D}(s)$}}};

\end{tikzpicture}
%\end{document}


==> ext_patch.tex <==
%\documentclass[tikz,border=3mm]{standalone}
%\begin{document}

\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}]
\pgfmathsetmacro{\factor}{1/sqrt(2)};
\coordinate  (A) at (2,0,-1*\factor);
\coordinate  (B) at (2.2,-1.2,2*\factor);
\coordinate  (C) at (-0.5,1,2*\factor);
\coordinate  (D) at (0.5,-2,2*\factor);
\coordinate  (E) at (0.5,3.5,3*\factor);
\coordinate  (F) at (0.8,2.8,-2*\factor);
\coordinate  (G) at (-1.2,-1,2*\factor);
\coordinate  (H) at (5.7,-0.5,5*\factor);
\coordinate  (I) at (1,-0.25,5*\factor);
\coordinate  (L) at (-2.5,3.2,-2.1*\factor);
\coordinate  (M) at (4.5,3,0*\factor);
\coordinate  (N) at (3.5,0.4,-1*\factor);
\coordinate  (O) at (2,3,-3.5*\factor);
\coordinate  (P) at (2.6,2.6,-2*\factor);
%\draw[->] (0,0) -- (3,0,0) node[right] {$x$};
%\draw[->] (0,0) -- (0,3,0) node[above] {$y$};
%\draw[->] (0,0) -- (0,0,3) node[below left] {$z$};
%\foreach \i in {A,B,C,D}
%\draw[dashed] (0,0)--(\i);
\draw[black, fill=white!90!gray] (A)--(D)--(C)--cycle;
\draw[black,  fill=gray!60!] (A) --(B)--(D)--cycle;
\draw[black, fill=gray!60!] (E) --(C)--(A)--cycle;
\draw[black,   fill=gray!60!] (E) --(F)--(A)--cycle;
\draw[black,    fill=gray!60!] (B) --(A)--(H)--cycle;
\draw[black,    fill=gray!60!] (C) --(G)--(I)--cycle;
\draw[black, fill=white!90!gray] (C) -- (E) -- (F)--(L)--cycle;
\draw[black,  fill=white!90!gray] (A) --(F)--(M)--cycle;
\draw[black,   fill=gray!60!] (A) --(N)--(M)--cycle;
\draw[black,    fill=gray!60!] (A) --(N)--(H)--cycle;
\draw[black,    fill=gray!60!] (F) --(O)--(P)--cycle;
%\draw[-, fill=gray!30!blue, opacity=.2] (E) --(G)--(H)--cycle;
\node [font=\Large, right] at (3, -2.2) {$\omega_j$};


%cylinder Gamma
\draw[dashed, very thick] (1, 5) ellipse (1.5 and 0.3);
\draw[dashed, very thick] (1, -3) ellipse (1.5 and 0.3);
\draw[black, very  thick] (-0.5, 3.6) -- (-0.5, 6);
\draw[black, very thick, opacity=.2] (-0.5, 3.6) -- (-0.5, -1.6);
\draw[black, very  thick] (-0.5, -1.6) -- (-0.5, -4); 
\draw[ very thick] (2.5, 6) -- (2.5, 3.2);
\draw[ very thick, opacity =0.2] (2.5, 3.2) -- (2.5, -1.8);
\draw[very thick] (2.5, -1.8) -- (2.5, -4);
\node [font=\Large, right] at (-1.3, 5) {$\Gamma$};

%centerline \Lambda
\draw[very thick] (1, 6) -- (1, 3.2);
\draw[red, very thick, opacity=.4] (1, 3.2) -- (1, -1.8);
\draw[very thick, ]  (1, -1.7) -- (1, -4);
\node [font=\Large, right] at (1.1, 4.2) {$\Lambda$};
\node [font=\Large, right] at (1.1, 4.2) {$\Lambda$};
\node [font=\Large, right, red] at (-0.7, -0.2) {$\omega _j \cap \Lambda$};
\end{tikzpicture}



%\end{document}

==> gamma_generated.tex <==
%\documentclass[tikz,border=3mm]{standalone}
%\usetikzlibrary{calc}
%\usetikzlibrary{shapes, snakes, patterns, arrows}
%\begin{document}

\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}]
\pgfmathsetmacro{\factor}{1/sqrt(2)};


\coordinate  (A) at (-2.5,1.5,-2.1*\factor);
\coordinate  (B) at (3.8,4,0*\factor);
\coordinate  (C) at (3.6,-2,2*\factor);
\coordinate  (D) at (6.5,2.7,8*\factor);
\draw[thick, black,    fill=white!90!gray, opacity=1] (A) --(B)--(C)--cycle;
\draw[ thick,black,  fill=gray!60!, opacity=0.7] (D) --(B)--(C)--cycle;
\draw[thick,gray!60!] (D) --(A);
\node [font=\Large, right] at (3.5, -2.5) {$\omega_j $};


%cylinder Gamma
%\draw[dashed, very thick] (1, 5) ellipse (1.5 and 0.3);
%\draw[dashed, very thick] (1, -3) ellipse (1.5 and 0.3);
\draw[black, very  thick] (-0.5, 2.55) -- (-0.5, 5);
\draw[black, very thick, opacity=.2] (-0.5, 2.55) -- (-0.5, 0.75);
\draw[black, very  thick] (-0.5, 0.75) -- (-0.5, -3); 
\draw[ very thick] (2.5, 5) -- (2.5, 3.55);
\draw[ very thick, opacity =0.2] (2.5, 3.55) -- (2.5, -2);
\draw[very thick] (2.5, -2) -- (2.5, -3);
\node [font=\Large, right] at (-1.2, 4.5) {$\Gamma$};


%centerline \Lambda
\draw[very thick] (1, 5) -- (1, 3.05);
\draw[red, very thick, opacity=.6] (1, 3.05) -- (1, -0.65);
\draw[very thick, ]  (1, -0.65) -- (1, -3);
\node [font=\Large, right] at (1.1, 3.8) {$\Lambda$};
\node [font=\Large, right, red] at (1, 0.4) {$\omega _j \cap \Lambda$};

\draw[dashed, very thick, purple, opacity=.4] (1, 3.05) ellipse (1.5 and 0.3);
\draw[dashed, very thick, purple, opacity=.4] (1, -0.65) ellipse (1.5 and 0.3);

\fill [purple, opacity=0.3]  (-0.5, -0.65) arc (180:360:1.5 and 0.3) -- (2.5, 3.05) arc (0:180:1.5 and -0.3);
\node [font=\Large, right, purple] at (-2, 0) {$\Gamma_{\omega_j \cap \Lambda}$};

\end{tikzpicture}

%\end{document}

==> intersection.tex <==
%\documentclass[tikz,border=3mm]{standalone}
%\usetikzlibrary{calc}
%\usetikzlibrary{shapes, snakes, patterns, arrows}
%\begin{document}
\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}]

\pgfmathsetmacro{\factor}{1/sqrt(2)};

%tetrahedron
\coordinate  (A) at (-2.5,1.5,-2.1*\factor);
\coordinate  (B) at (3.8,4,0*\factor);
\coordinate  (C) at (3.6,-2,2*\factor);
\coordinate  (D) at (6.5,2.7,8*\factor);
\draw[thick, black,    fill=white!90!gray, opacity=1] (A) --(B)--(C)--cycle;
\draw[ thick,black,  fill=gray!60!, opacity=0.7] (D) --(B)--(C)--cycle;
\draw[thick,gray!60!] (D) --(A);
\node [font=\Large, right] at (3.5, -2.5) {$\omega_j $};


%cylinder Gamma
%\draw[dashed, very thick] (1, 5) ellipse (1.5 and 0.3);
%\draw[dashed, very thick] (1, -3) ellipse (1.5 and 0.3);
\draw[black, very  thick] (-0.5, 2.55) -- (-0.5, 5);
\draw[black, very thick, opacity=.2] (-0.5, 2.55) -- (-0.5, 0.75);
\draw[black, very  thick] (-0.5, 0.75) -- (-0.5, -3); 
\draw[ very thick] (2.5, 5) -- (2.5, 3.55);
\draw[ very thick, opacity =0.2] (2.5, 3.55) -- (2.5, -2);
\draw[very thick] (2.5, -2) -- (2.5, -3);
\node [font=\Large, right] at (-1.2, 4.5) {$\Gamma$};

%centerline \Lambda
\draw[very thick] (1, 5) -- (1, 3.05);
\draw[red, very thick, opacity=.6] (1, 3.05) -- (1, -0.65);
\draw[very thick, ]  (1, -0.65) -- (1, -3);
\node [font=\Large, right] at (1.1, 3.8) {$\Lambda$};
\node [font=\Large, right, red] at (1, 0.4) {$\omega _j \cap \Lambda$};

%intersection
\draw[dashed, very thick, purple, opacity=.4] (1, 3.05) ellipse (1.5 and 0.3);
\draw[dashed, very thick, purple, opacity=.4] (1, -0.65) ellipse (1.5 and 0.3);
\draw[dashed, very thick, purple, opacity=.4] (1, 1.5) ellipse (1.5 and 0.3);
\fill [purple, opacity=0.3]  (2.5, -0.65) arc (360:280:1.5 and 0.3) -- (-0.5, 0.75) -- (-0.5, 2.55) -- (0.3, 2.8) arc (118:0:1.5 and -0.3);
\node [font=\Large, right, purple] at (-2, -0.1) {$\Gamma_{\omega_j \cap \Lambda} \cap \omega_j$};

\end{tikzpicture}

%\end{document}
